Learning Real Facial Concepts for Independent Deepfake Detection

Deepfake detection models often struggle with generalization to unseen datasets, manifesting as misclassifying real instances as fake in target domains. This is primarily due to an overreliance on forgery artifacts and a limited understanding of real faces. To address this challenge, we propose a novel approach RealID to enhance generalization by learning a comprehensive concept of real faces while assessing the probabilities of belonging to the real and fake classes independently. RealID comprises two key modules: the Real Concept Capture Module (RealC2) and the Independent Dual-Decision Classifier (IDC). With the assistance of a MultiReal Memory, RealC2 maintains various prototypes for real faces, allowing the model to capture a comprehensive concept of real class. Meanwhile, IDC redefines the classification strategy by making independent decisions based on the concept of the real class and the presence of forgery artifacts. Through the combined effect of the above modules, the influence of forgery-irrelevant patterns is alleviated, and extensive experiments on five widely used datasets demonstrate that RealID significantly outperforms existing state-of-the-art methods, achieving a 1.74% improvement in average accuracy.

==> sec/3_motivation.tex <==
\section{Why are the real misclassified as fake?}

To improve the generalization performance in the target domain, we attribute the misclassification of real samples to two causes and analyze them separately.

\begin{center}
\noindent\fbox{\parbox{0.95\linewidth}
{\textbf{Hypothesis 1 - The limited `Real Concept':} The homogeneous real features limit the learning of `Real Concept' and the real samples that fall outside the learned concept are prone to be misclassified.}
}
\end{center}

By comparing the distribution of the real data in Figure~\ref{fig:tsne1}(c)-(d), we find that the test data within the overlapping areas of the training data can be classified as true negatives. In contrast, the data outside the overlap areas are misclassified as false positives. We reasonably infer that the distribution range of the training data is strongly correlated with the generalization performance.


\begin{center}
\noindent\fbox{\parbox{0.95\linewidth}
{\textbf{Hypothesis 2 - The reliance on Fake Traces:} The difficulty in learning `Real Concept' leads to heavy reliance on forgery traces and misclassification of real samples with `mis-artifacts.'}
}
\end{center}

\begin{figure}[t]
\centering
\includegraphics[width=7.5cm]{sec/Image/cam/cam-1.pdf}
\caption{A comparison of the heatmaps.}
\label{fig:cam-1}
\end{figure}

Observing the high-response areas in Figure \ref{fig:cam-1}, we find that the model focuses on global characteristics for true negatives but relies on local features for true positives and false positives whose high-response areas exhibit consistent characteristics such as blurriness, jitter, and abrupt transitions. We refer to these characteristics, which are highly correlated with forgery data but may also appear in misclassified real data, as `mis-artifact.' Meanwhile, we infer that when the model detects any mis-artifacts, it is likely to arbitrarily classify the input as fake.


==> sec/7_authorbio.tex <==






\noindent
\parbox[t]{0.1\textwidth}{%
    \includegraphics[width=0.1\textwidth]{sec/author_img/Harry_Cheng.jpg}% 替换为你的图片
}%
\hfill
\parbox[t]{0.4\textwidth}{%
{Harry Cheng} received the B.Eng. and master degree from Shandong University, China, in 2018 and 2021, respectively. He is currently pursuing the Ph.D. degree with the School of Computer Science and Technology, Shandong University, under the supervision of Liqiang Nie. His research interests include Deepfake detection and multi-modal computing.
}
